Evolving Loop Programs: Discovering How Frozen Transformers Should Loop

Reusing transformer blocks through loops can improve pretrained models without updating their weights. However, useful loops require coordinated choices about which blocks repeat, how hidden states evolve, and when computation is reused. We introduce Evolving Loop Programs (ELP), an offline LLM-based method for discovering executable inference programs with favorable quality-compute trade-offs. The search jointly edits loop structure, state-update dynamics, and execution controls, including sampling schedules, guidance, and intermediate-state reuse. The LLM writes diagnostic code and combines observations of model behavior with accumulated development evaluations to guide these edits. We retain nondominated programs for different operating priorities, then freeze their code and parameters. During deployment, these programs execute their loops without further calls to the search LLM. Experiments span image, video, and text using separately searched programs. For images, diffusion transformers trained with and without loops achieve better quality-compute trade-offs. A selected RAE program improves GenEval and DPG-Bench with a $5.19\times$ FLOPs speedup over standard unlooped inference. On Looped-DiT, both improve at equal or lower compute than native inference with matched sampling steps. For video, frozen programs improve long-video consistency across LongLive and Self-Forcing without weight updates. To the best of our knowledge, this is the first empirical validation of training-free transformer-block looping in pretrained video world models. For text, programs improve aggregate reasoning accuracy on Qwen3-4B. Our code will be released.

==> reference-names.tex <==
\makeatletter
\AtBeginDocument{%
  \@ifpackageloaded{cleveref}{%
    \crefname{figure}{Figure}{Figures}%
    \Crefname{figure}{Figure}{Figures}%
    \crefname{table}{Table}{Tables}%
    \Crefname{table}{Table}{Tables}%
    \crefname{algorithm}{Algorithm}{Algorithms}%
    \Crefname{algorithm}{Algorithm}{Algorithms}%
    \crefname{algocf}{Algorithm}{Algorithms}%
    \Crefname{algocf}{Algorithm}{Algorithms}%
    \crefname{equation}{Equation}{Equations}%
    \Crefname{equation}{Equation}{Equations}%
    \crefname{section}{Section}{Sections}%
    \Crefname{section}{Section}{Sections}%
    \crefname{subsection}{Section}{Sections}%
    \Crefname{subsection}{Section}{Sections}%
    \crefname{subsubsection}{Section}{Sections}%
    \Crefname{subsubsection}{Section}{Sections}%
    \crefname{appendix}{Appendix}{Appendices}%
    \Crefname{appendix}{Appendix}{Appendices}%
    \crefname{chapter}{Chapter}{Chapters}%
    \Crefname{chapter}{Chapter}{Chapters}%
    \crefname{listing}{Listing}{Listings}%
    \Crefname{listing}{Listing}{Listings}%
  }{}%
  \@ifpackageloaded{hyperref}{%
    \def\figureautorefname{Figure}%
    \def\tableautorefname{Table}%
    \def\algorithmautorefname{Algorithm}%
    \def\algocfautorefname{Algorithm}%
    \def\equationautorefname{Equation}%
    \def\sectionautorefname{Section}%
    \def\subsectionautorefname{Section}%
    \def\subsubsectionautorefname{Section}%
    \def\appendixautorefname{Appendix}%
    \def\chapterautorefname{Chapter}%
    \def\listingautorefname{Listing}%
  }{}%
}
\makeatother


==> sec/table_replay_settings.tex <==
\begin{table*}[!htbp]
\centering
\caption{\textbf{Replay uses fixed sampling and numerical settings within each frozen backbone.} Panel (a) lists execution settings; (b) identifies the native and loop references used for compute comparisons.}
\label{tab:supp_repro_details}
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.10}
\textbf{(a) Inputs, sampling, and execution.}\par\smallskip
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}%
>{\raggedright\arraybackslash}p{0.175\textwidth}%
>{\raggedright\arraybackslash}p{0.205\textwidth}%
>{\raggedright\arraybackslash}p{0.210\textwidth}%
>{\raggedright\arraybackslash}p{0.235\textwidth}%
>{\raggedright\arraybackslash}p{0.115\textwidth}@{}}
\toprule
\textbf{Backbone} & \textbf{Input / decoding} & \textbf{Samples / seeds} & \textbf{Precision / batch} & \textbf{GPUs} \\
\midrule
\multicolumn{5}{@{}l}{\textbf{Image generation}} \\
Scale-RAE~\cite{tong2026scaling} &
$224\times224$; DPG crop $224$ &
$1$/prompt; seed $42$ &
BF16 AMP; FP32 decode; batch $8$ &
$1\times$ RTX~5090 \\
\addlinespace[2pt]
RAE~\cite{leng2026diffusionbench} &
$256\times256$; DPG crop $256$ &
$1$/prompt; seed $42$ &
BF16 AMP; FP32 decode; batch $16$ &
$1\times$ RTX~5090 \\
\addlinespace[2pt]
Looped-DiT-B32~\cite{chng2026looped} &
$512\times512$; DPG crop $512$ &
$4$ seeds/prompt; seed $0$; $8$ GPU RNGs &
BF16 AMP; batch $16$ prompts ($64$ images) &
$32\times$ H100 \\
\midrule
\multicolumn{5}{@{}l}{\textbf{Text reasoning and generation}} \\
Qwen3-4B~\cite{yang2025qwen3} &
Multiple-choice log-likelihood &
$1$/question; zero-shot; seed $1234$ &
BF16, SDPA; batch $8$ &
$1\times$ RTX~5090 \\
\addlinespace[2pt]
Dory1.0-4B~\citesupp{fishman2026dory} &
STEM: log-likelihood\newline Open: generation &
STEM: $1$/question, zero-shot, seed $1234$\newline Open: $8$/prompt &
STEM: BF16, batch $8$\newline Open: BF16, $16$ seqs/GPU &
STEM: $16\times$ H100\newline Open: $32\times$ H100 \\
\midrule
\multicolumn{5}{@{}l}{\textbf{Video generation}} \\
LongLive~2.0 5B~\cite{chen2026longlive2} &
$1280\times704$; $379$ frames at $24$\,fps &
$1$/scene; official per-scene seeds &
BF16; $1$ scene/GPU &
$32\times$ H100 \\
\addlinespace[2pt]
LongLive~2.0 5B ($60$\,s MemFlow) &
$1280\times704$; $1{,}437$ frames at $24$\,fps ($45{\times}8$ chunks) &
$1$/narrative; $6{\times}10$\,s prompts &
BF16; $1$ video/GPU &
$32\times$ H100 \\
\addlinespace[2pt]
LongLive~1.0 1.3B~\cite{yang2026longlive} &
$832\times480$; $379$ frames at $24$\,fps &
$1$/scene; official per-scene seeds &
BF16; $1$ scene/GPU &
$32\times$ H100 \\
\addlinespace[2pt]
Self-Forcing 1.3B~\cite{huang2025selfforcing} &
$832\times480$; $379$ frames at $24$\,fps &
$1$/scene; official per-scene seeds &
BF16; $1$ scene/GPU &
$32\times$ H100 \\
\addlinespace[2pt]
Wan2.1-1.3B~\cite{wan2025wan} &
$832\times480$; $81$ frames at $16$\,fps &
$1$/prompt; seed $42$ &
BF16 AMP; FP32 time/head/VAE; batch $1$/GPU &
$24\times$/$32\times$ H100 \\
\bottomrule
\end{tabular*}

\medskip
\textbf{(b) Native configurations and compute references.}\par\smallskip
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}%
>{\raggedright\arraybackslash}p{0.175\textwidth}%
>{\raggedright\arraybackslash}p{0.550\textwidth}|%
>{\raggedright\arraybackslash}p{0.235\textwidth}@{}}
\toprule
\textbf{Backbone} & \textbf{Reference configuration} & \textbf{Compute} \\
\midrule
Scale-RAE &
$25$-step Base, guidance $1.0$; Loop + LG: blocks $12$--$27$, $K=4$, LG $2.8$ &
Base: $31.58$\,TFLOPs\newline Loop + LG: ${\approx}87.62$\newline Loop w/o LG: $56.04$ \\
\addlinespace[2pt]
RAE &
$50$-step Base; Loop + LG: blocks $15$--$22$, $K=4$, LG $9.0$ &
Base: $29.07$\,TFLOPs\newline Loop + LG: $54.20$\newline Loop w/o LG: $39.67$ \\
\addlinespace[2pt]
Looped-DiT-B32 &
$100$ Euler steps, $K=4$, CFG $6.0$, noise scale $2.0$ &
Full reference: $53.18$\,TFLOPs \\
\midrule
Qwen3-4B &
Standard inference; Fixed Loop uses Euler updates on layers $15$--$18$, $K=3$ &
FLOPs and latency not reported \\
\addlinespace[2pt]
Dory1.0-4B &
STEM: native $K\in\{2,3,4\}$\newline Open-ended: native $K\in\{2,4\}$ &
STEM: $11.03/14.74/18.44$\,GFLOPs/token\newline Open: $96{,}300/161{,}198$\,TFLOPs \\
\midrule
LongLive~2.0 5B &
No-loop, $4$-step chunk UniPC; shift $5$; steps $[999,937,833,624]$ &
Base: $7{,}621$\,TFLOPs\newline Ours: $13{,}716$ \\
\addlinespace[2pt]
LongLive~2.0 ($60$\,s MemFlow) &
No-loop, $4$-step chunk UniPC; shift $5$; $[999,937,833,624]$; $6$ prompt switches &
Base: $30{,}086$\,TFLOPs\newline Min.\ Speed: $26{,}766$\newline Matched Qual.: $32{,}493$ \\
\addlinespace[2pt]
LongLive~1.0 1.3B &
No-loop, $4$-step chunk denoising; steps $[1000,750,500,250]$ &
Base: $4{,}748$\,TFLOPs\newline Ours: $7{,}627$ \\
\addlinespace[2pt]
Self-Forcing 1.3B &
No-loop autoregressive chunk diffusion &
Base: $5{,}972$\,TFLOPs\newline Ours: $7{,}564$ \\
\addlinespace[2pt]
Wan2.1-1.3B &
$50$-step UniPC; shift $8.0$, CFG $6.0$; $30$-step control &
Base: $28{,}300$\,TFLOPs\newline Control: $16{,}980$ \\
\bottomrule
\end{tabular*}
\end{table*}

\paragraph{Software and rollout details.}
Table~\ref{tab:supp_repro_details} separates execution settings from the native compute references. Scale-RAE, RAE, and Wan retain checkpoint tensor dtypes under BF16 autocast. Qwen3-4B uses \texttt{torch 2.8.0} and \texttt{transformers 4.57.1} with \texttt{sdpa}; Dory STEM uses multiple-choice log-likelihood with \texttt{torch 2.7.1} and \texttt{transformers 4.57.6}. Dory open-ended generation uses \texttt{vLLM} with CUDA graphs and $8$ GPUs per candidate, temperature $1.0$, and top-$p$ $0.95$. RememBench videos last $15.79$\,s, with evaluation at frames $86$ and $378$; the $60$\,s MemFlow rollouts generate $45{\times}8$ latent chunks ($1{,}437$ decoded frames at $24$\,fps = $59.875$\,s). LongLive~2.0 uses $12\times8$ latent-frame chunks; LongLive~1.0 uses $32\times3$. Self-Forcing uses a $21$-frame attention window. Wan videos last $5.0625$\,s.


==> sec/table_search_settings.tex <==
\begin{table*}[!htbp]
\centering
\caption{\textbf{Search settings vary by backbone, edit scope, and objective.} Split counts are development / validation / full; Wan's validation split includes $16$ previously agent-visible videos. Anchors are measured unless marked synthetic. Initial context $\mathcal{C}_0$: video and world-model searches use Minimal context (except the Matched and Library-only $60$\,s regimes), while image and text-reasoning backbones mostly use Matched prior; $60$\,s LongLive~2.0 searches run $32$ candidates over $4$ rounds.}
\label{tab:supp_exp_settings}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}%
>{\raggedright\arraybackslash}p{0.215\textwidth}%
>{\raggedright\arraybackslash}p{0.095\textwidth}%
>{\raggedright\arraybackslash}p{0.170\textwidth}%
>{\raggedright\arraybackslash}p{0.175\textwidth}%
>{\raggedright\arraybackslash}p{0.070\textwidth}%
>{\raggedright\arraybackslash}p{0.185\textwidth}@{}}
\toprule
\textbf{Backbone / setting} & \textbf{LLM} & \textbf{Edit scope} & \textbf{Dev / Val / Full} & \textbf{Anchors} & \textbf{Search objectives} \\
\midrule
\rowcolor{gray!10}
\multicolumn{6}{@{}l@{}}{\textbf{Image generation}\quad GenEval ($553$) and DPG ($1{,}065$); counts in prompts} \\
Scale-RAE~\cite{tong2026scaling}: config. & \texttt{Astra} & Configuration; fixed probes & $320/1{,}298/1{,}618$ & 2 & GenEval, DPG, $s_{\mathrm{lat}}$ \\
Scale-RAE: main & \texttt{Astra} & Program + probes & $320/1{,}298/1{,}618$ & 2 & GenEval, DPG, $s_{\mathrm{lat}}$ \\
Scale-RAE: no diagnostics & \texttt{Astra} & Program; zero probes & $320/1{,}298/1{,}618$ & 2 & GenEval, DPG, $s_{\mathrm{lat}}$ \\
Scale-RAE: True & \texttt{Argon} & Program + probes & $320/1{,}298/1{,}618$ & 2 & GenEval, DPG, $s_{\mathrm{lat}}$ \\
Scale-RAE: Strong / Ultra & \texttt{Argon} & Program + probes & $320/1{,}298/1{,}618$ & 2 + 1 synthetic & Same; shifted target \\
Scale-RAE: GenEval-only & \texttt{Astra} & Program + probes & $112/441/553$ & 2 & GenEval only \\
Scale-RAE: DPG-only & \texttt{Astra} & Program + probes & $208/857/1{,}065$ & 2 & DPG only \\
\addlinespace[3pt]
RAE~\cite{leng2026diffusionbench} & \texttt{Astra} & Program + probes & $320/1{,}298/1{,}618$ & 3 & GenEval, DPG, $s_{\mathrm{lat}}$ \\
Looped-DiT-B32~\cite{chng2026looped} & \texttt{Argon} & Program + probes & $320/1{,}298/1{,}618$; four seeds & 4 & GenEval, DPG, $s_{\mathrm{lat}}$ (cap $8\times$) \\
\midrule
\rowcolor{gray!10}
\multicolumn{6}{@{}l@{}}{\textbf{Text reasoning}\quad STEM suite: $4{,}145$ questions; open-ended suite: $563$ tasks} \\
Qwen3-4B~\cite{yang2025qwen3}: True & \texttt{Argon} & Program + probes & $829/3{,}316/4{,}145$ & 2 & Five quality metrics; no cost \\
Qwen3-4B: Mild / Strong / Extreme & \texttt{Argon} & Program + probes & $829/3{,}316/4{,}145$ & 2 + 1 synthetic & Same; shifted target \\
Dory1.0-4B~\citesupp{fishman2026dory}: open-ended & \texttt{Carbon} & Program + probes; transitions, KV reuse & $113/450/563$; eight runs/prompt & 2 & Accuracy, time, FLOPs; $K{=}2$ \\
Dory1.0-4B: STEM & \texttt{Carbon} & Program + probes; depth, transitions & $829/3{,}316/4{,}145$ & 1--2 & Quality--compute at matched $K\!\in\!\{2,3,4\}$ \\
\midrule
\rowcolor{gray!10}
\multicolumn{6}{@{}l@{}}{\textbf{Long-video generation}\quad RememBench ($100$ scenes) and MemFlow ($100$ $60$\,s videos)} \\
LongLive~2.0 5B~\cite{chen2026longlive2} & \texttt{Astra} & Block-scoped program + probes & $20/80/100$ & 1 & CLIP, $1/(1+\mathrm{LPIPS})$ \\
LongLive~1.0 1.3B~\cite{yang2026longlive} & \texttt{Astra} & Block-scoped program + probes & $20/80/100$ & 1 & Same quality pair \\
Self-Forcing 1.3B~\cite{huang2025selfforcing} & \texttt{Astra} & Program + probes; AST loop API & $20/80/100$ & 1 & Same quality pair \\
LongLive~2.0 5B: $60$\,s context ($4$ regimes) & \texttt{Argon} & Program + probes ($2{\times}2\;\mathcal{C}_0$) & $20/80/100$ & 1 & 5D: Quality, Cons., CLIP mean/min, $s_{\mathrm{lat}}$ \\
LongLive~2.0 5B: $60$\,s fixed-sched. & \texttt{Argon} & Fixed-schedule loop rule; fixed probes & $20/80/100$ & 1 & 3D: Quality, Cons., CLIP mean; no cost \\
\midrule
\rowcolor{gray!10}
\multicolumn{6}{@{}l@{}}{\textbf{Short-video generation}\quad Local VBench-1.0 ($16$ dimensions); counts in videos} \\
Wan2.1-1.3B~\cite{wan2025wan}: Speed / Balanced & \texttt{Astra} & Program + probes & $48/208/256$ & 1 & Quality, Semantic, latency \\
Wan2.1-1.3B: Quality / Quality-alt. & \texttt{Argon} & Program + probes & $48/208/256$ & 1 & Quality, Semantic, Total; no cost \\
\bottomrule
\end{tabular*}
\end{table*}

